LF Tracy: A Unified Single-Pipeline Approach for Salient Object Detection in Light Field Cameras

Leveraging rich information is crucial for dense prediction tasks. Light field (LF) cameras are instrumental in this regard, as they allow data to be sampled from various perspectives. This capability provides valuable spatial, depth, and angular information, enhancing scene-parsing tasks. However, we have identified two overlooked issues for the LF salient object detection (SOD) task. (1): Previous approaches predominantly employ a customized two-stream design to discover the spatial and depth features within light field images. The network struggles to learn the implicit angular information between different images due to a lack of intra-network data connectivity. (2): Little research has been directed towards the data augmentation strategy for LF SOD. Research on inter-network data connectivity is scant. In this study, we propose an efficient paradigm (LF Tracy) to address those issues. This comprises a single-pipeline encoder paired with a highly efficient information aggregation (IA) module (around 8M parameters) to establish an intra-network connection. Then, a simple yet effective data augmentation strategy called MixLD is designed to bridge the inter-network connections. Owing to this innovative paradigm, our model surpasses the existing state-of-the-art method through extensive experiments. Especially, LF Tracy demonstrates a 23% improvement over previous results on the latest large-scale PKU dataset. The source code is publicly available at: https://github.com/FeiBryantkit/LF-Tracy.

==> Tab/Tab6.tex <==
\begin{wraptable}{l}{0.48\textwidth}
\vspace{-1em}
    \centering
    \renewcommand{\arraystretch}{1.5}
        \setlength{\tabcolsep}{1.5mm}
        \begin{tabular}{c:c:c:c:c}
        \toprule[0.5mm]
        \textbf{Stack Size} & \textbf{2} & \textbf{3} & \textbf{5} & \textbf{12}\\ 
        \midrule
        \textbf{w/o. IA} & .137 & .141 & .205 & .332 \\
        \textbf{w. IA} & .051 & .051 & .049 & \red{.046} \\
        \bottomrule
        \end{tabular}
        \caption{An ablation study for the IA Module is conducted to evaluate its capabilities in terms of feature fusion and alignment.}
        \label{tab:521}
\end{wraptable}

\begin{wraptable}{l}{0.48\textwidth}
    \centering
    \setlength{\tabcolsep}{1mm}
    \begin{tabular}{c:c:c:c:c}
    \toprule[0.5mm]
    \textbf{F\&S} & \textbf{A\&PD} & \textbf{DA} & \textbf{ADD} & \textbf{A\&D}\\ 
    \midrule
    \textbf{MAE} & .046 & .056 & \textcolor{red}{.332} & \textcolor{blue}{.048} \\
    \bottomrule
    \end{tabular}
    \caption{The exploration of different fusion strategies involved testing four methods: A\&PD represents attention and dot product (with learnable parameters), DA represents deformable cross attention, ADD represents addition, and A\&D represents attention and addition.}
    \label{tab:522}
\end{wraptable}

\begin{wraptable}{r}{0.48\textwidth}
    \centering
    \setlength{\tabcolsep}{1.5mm}
    \begin{tabular}{c:c:c:c:c}
    \toprule[0.5mm]
    \textbf{R\&Rate} & \textbf{0} & \textbf{4} & \textbf{8} & \textbf{16}\\ 
    \midrule
    \textbf{MAE} & .050 & .049 & .046 & .050 \\
    \bottomrule
    \end{tabular}
    \caption{In the first step of the IA Module, the reduction rate for the dimensions of Query and Key is evaluated. We utilize four different parameters: no compression, one-quarter compression, one-eighth compression, and one-sixteenth compression. The MAE and GFlops are reported. `R\&Rate' indicates Reduction Rate.}
    \label{tab:523}
\end{wraptable}


==> Tab/Tab7.tex <==
\begin{table}
\vspace{-2em}
  \centering
  \scriptsize
  \setlength{\tabcolsep}{1mm}
    \begin{tabular}{c:c:c:c:c}
    \toprule[0.5mm]
    \textbf{F\&S} & \textbf{A\&PD} & \textbf{DA} & \textbf{ADD} & \textbf{A\&D}\\ 
    \midrule
    \textbf{MAE} & .046 & .056 & \red{.332} & \revised{.048} \\
    \bottomrule
    \end{tabular}
    \label{tab:T5}
    \vspace{-0.5em}
    \caption{Results for various studies. ``w/o.'' is the abbreviation for ``without''. ``w.'' is the abbreviation for ``with''. MAE is reported.}
    \vspace{-2em}
\end{table}
